Measuring the Redundancy of Information from a Source Failure Perspective

In this paper, we define a new measure of the redundancy of information from a fault tolerance perspective. The partial information decomposition (PID) emerged last decade as a framework for decomposing the multi-source mutual information $I(T;X_1, ..., X_n)$ into atoms of redundant, synergistic, and unique information. It built upon the notion of redundancy/synergy from McGill's interaction information (McGill 1954). Separately, the redundancy of system components has served as a principle of fault tolerant engineering, for sensing, routing, and control applications. Here, redundancy is understood as the level of duplication necessary for the fault tolerant performance of a system. With these two perspectives in mind, we propose a new PID-based measure of redundancy $I_{\text{ft}}$, based upon the presupposition that redundant information is robust to individual source failures. We demonstrate that this new measure satisfies the common PID axioms from (Williams 2010). In order to do so, we establish an order-reversing correspondence between collections of source-fallible instantiations of a system, on the one hand, and the PID lattice from (Williams 2010), on the other.

==> Sections/conclusion.tex <==
\section{Concluding Thoughts}

In this work, we introduced a new measure for the redundancy of information, inspired by the operational use of redundancy from the fault tolerance literature.
Our measure fits within the broader partial information decomposition (PID) field, while contributing a novel perspective to redundancy as conceived by PID.
We have provided a simple example in Sec.~\ref{sec:example}, and began sketching a more general operational interpretation of our redundancy function in the last section.
We intend to expand upon this operational interpretation in future.
There is a game-theoretic interpretation of $\Ift$ as we have defined it in this paper, in which players' actions include the selection and sabotage of information assets.
